MultiPL-E: A Scalable and Extensible Approach to Benchmarking Neural Code Generation

Large language models have demonstrated the ability to generate both natural language and programming language text. Such models open up the possibility of multi-language code generation: could code generation models generalize knowledge from one language to another? Although contemporary code generation models can generate semantically correct Python code, little is known about their abilities with other languages. We propose MultiPL-E, a system for translating unit test-driven code generation benchmarks to new languages. We create the first massively multilingual code generation benchmark by using MultiPL-E to translate two popular Python code generation benchmarks to 18 additional programming languages. We use MultiPL-E to extend the HumanEval benchmark and MBPP benchmark to 18 languages that encompass a range of programming paradigms and popularity. Using these new parallel benchmarks, we evaluate the multi-language performance of three state-of-the-art code generation models: Codex, CodeGen, and InCoder. We find that Codex matches or even exceeds its performance on Python for several other languages. The range of programming languages represented in MultiPL-E allow us to explore the impact of language frequency and language features on model performance. Finally, the MultiPL-E approach of compiling code generation benchmarks to new programming languages is both scalable and extensible, making it straightforward to evaluate new models, benchmarks, and languages.

==> carolyn-related-work.tex <==
\section{Related work}

\subsection{Models for Programming Language tasks}
CodeBERT\cite{feng2020codebert}

PyMT5\cite{clement-etal-2020-pymt5}

%datasets
\subsubsection{\citet{raffel2019exploring}: Colossal Clean Crawled Corpus}

\subsubsection{\citet{thepile}: The Pile}

\subsection{LLMs that test code generation}

\subsubsection{\citet{brown2020language}: GPT-3}

\subsubsection{GPT-J}

\subsubsection{GPT-Neo}

\subsubsection{GPT-Neo-X}

\subsection{LLMs Fine-tuned for Code generation}

\paragraph*{LLMs for NL2Code} 
Several models are trained for NL2Code tasks~\citet{chen2021evaluating, fried2022incoder, xu2022systematic, salesforce-codegen}.
Codex~\cite{chen2021evaluating} is a 12B parameter version of GPT-3 model fine-tuned on 159GB of deduped filtered Python code from Github. Codex samples tokens until it encounter one of the given stop sequences.
Codex is evaluated on HumanEval dataset by taking 200 samples for each pass@k metric.
InCoder~\cite{fried2022incoder} is a 6.7B parameter language model trained on 159GB of total data with 52GB of Python data, 57GB of Stackoverflow data from The Pile dataset~\cite{thepile}, and the remaining data from Github.
InCoder is evaluated using HumanEval and MBPP. 

\subsubsection{\citet{chen2021evaluating}: Codex} 

Fine-tuned GPT-3 model on 159 GB of deduped, filtered code. Code lexer is based on GPT-3 text tokenizer, extended with a set of tokens for representing different whitespace lengths.

Samples tokens until they encounter one of 5 stop sequences: `$\backslash$nclass', `$\backslash$ndef', `$\backslash$n\#', `$\backslash$nif', or
`$\backslash$nprint'. Uses nucleus sampling with p=0.95 for all samples. Finds the optimal temperature for pass@1 is 0,2, while pass@100 is 0.8.

Evaluates on HumanEval using pass@k metrics. They take 200 samples for each pass@k metric, regardless of k. 

Also report Codex-S, which is fine-tuned on problems from competitive programming websites (10,000) and from repos with CI (40,000).

Some error patterns they notice: long docstrings are hard; invoking undefined functions/variables; binding.

\subsubsection{\citet{fried2022incoder}: InCoder}

Trained on a causal masking objective: a sequence is replaced by a sentinel token and moved to the end of the sequence, training it to predict completions for missing regions. This also allows to it generate: you just don't add sentinel tokens.

Trained on 159 GB of data, 52 GB of it in Python. 57 GB are from StackOverflow (via The Pile) and the rest from GitHub. 

Allows tokens to extend over whitespace.

Trains a Transformer language model with 6.7B parameters.

Creates two evaluation datasets from HumanEval: a single line infilling and a multi-line infilling. 

Evaluates against prior work using HumanEval and MBPP. For HumanEval, samples 200 candidates and calculates pass@1 with temp=0.2, and pass@10 and pass@100 with temp=0.8. Uses top-p sampling with p=0.95 for all. 

Also tests on other tasks: type inference, variable name prediction, docstring generation. Evaluation datasets mostly taken from CodeXGLUE.

\subsubsection{\cite{xu2022systematic}: PolyCoder}

Claims to be the first language ``trained exclusively on code from multiple programming languages.'' This is dubious.

GPT-2 model with 2.7B parameters trained on most popular Github repos for 12 languages, taking only 25,000 repos per language.

Outperforms Codex in perplexity on C. In every other measure, less good.

Uses the same evaluation metrics as \citet{chen2021evaluating}, except weirdly they only sample 100 times. \molly{and they don't mention why!}

\subsubsection{Salesforce Codegen \cite{salesforce-codegen}}

\subsection{Code generation tasks}

NL2Code: generating code from docstring / natural language description.

Docstring generation: generate a docstring from a function.

\citet{tufano2020unit} generate unit tests from code.

\citet{lu2021codexglue} proposes 10 tasks.

\subsection{NL2Code benchmarks}

\subsubsection{\citet{chen2021evaluating}: HumanEval}. Proposes a benchmark dataset of 164 original programming problems with unit tests. The problems cover algorithms, simple mathematics, and language comprehension. Has an average of 7.7 tests per problem.

\subsubsection{\citet{hendrycks2021measuring}: APPS}. 5000 training and 5000 test examples of coding problems, each with a set of unit tests. Most involve full programs rather than generating individual functions. Average number of test cases per problem: 21.2.

Taken from websites where programmers share programming challenge problems. Problems are grouped by difficulty into introductory level, interview level, and competition level.

Two formats: call-based format where the programmer is given the beginning of a function, and standard input format, where the program must output its answers to the STDOUT stream (like ACM programming contest).

Computes the average number of tests passed. 

\molly{cites other dataset collections that they see as working on a similar problem: SPoC (below), Iyer \cite{iyer2018mapping} (Java), Spider (EMNLP) (SQL), \citet{raychev2016probabilistic} (JavaScript \& Python), }

\ca{\citet{raychev2016probabilistic} seems to be code generation without a natural language component-- they train the model to predict a missing AST node.}

\subsubsection{\citet{austin2021program}: MBPP and MathQA-Python}

Mostly Basic Programming Problems (MBPP): 974 Python functions, paired with natural language descriptions and test cases. Designed not to involve libraries or print statements. Each has 3 test cases. Most natural language descriptions are only 1 line.

MathQA-Python: 23,914 pairs of Python programs and natural language descriptions. The programs are in a strange format, since the prompts are taken from mathematical word problems with multiple choice answers.

Each problem contains three I/O examples as assert statements in the prompt.

They include the test cases in the prompt. They also report results from including 0, 1, 2, or 3 test cases.

\subsubsection{\citet{kulal2019spoc}: SPoC}

C++ code generation dataset. Uses crowdsourced descriptions of a line of code rather than documentation.

\subsection{Other code generation benchmarks}

In addition to code generation benchmarks that pair natural language comments with code, there are benchmarks that pair programming-related natural language questions with code snippets. These benchmarks include CoNaLa \citet{yin2018learning}, which mines matching natural language questions and code snippets from StackOverflow; \citet{husain2019codesearchnet}... 

\subsubsection{\citet{yin2018learning}: CoNaLa}

A dataset of natural language questions about code mined from StackOverflow. Pairs natural language intent with code snippet. Contains both a manually annotated subset and a larger automatically mined corpus.

\subsubsection{\citet{wang2022mconala}: MCoNaLa}

Translation of CoNaLa into Spanish, Japanese, and Russian.

\citet{husain2019codesearchnet}: benchmark for retrieving relevant code from natural language query.

\citet{lu2021codexglue}: benchmarks for 10 tasks.

\citet{villmow-etal-2021-contest}: benchmark for unit test generation.

\subsection{NL2Code evaluation}

\citet{xu2022in-ide}

\subsubsection{\citet{xu2022systematic}}

Evaluates Codex, GPT-J, GPT-Neo, GPT-NeoX-20B, Code-
Parrot and proposes a new model, PolyCoder. Evaluates on HumanEval, and also looks at perplexity in 12 languages: C, C\#, C++, Go, Java, JavaScript, PHP, Python, Ruby, Rust, Scala, TypeScript.

\subsubsection{\citet{austin2021program}}

Evaluates Transformer models on MBPP and MathQA-Python. The largest has 137B parameters.

Runs a fine-tuning experiment as well as a prompt engineering experiment where they prepend some solved problems to the front of the prompt. 

Evaluates using pass@80 with temperature of 0.5. Also measures the fraction of samples that pass all tests.

Breaks errors into multiple categories: syntax errors, type errors, runtime errors, and tests failed.

Also investigates whether the largest model can predict the output from a function call. It generally cannot.

\subsection{Metric citations}

Pass@k comes from \citet{kulal2019spoc}.

\citet{hendrycks2021measuring} use average number of test cases passed, in addition to pass@1, pass@5, and pass@100.

\citet{kulal2019spoc} evaluates using unit tests.

\citet{chen2021evaluating} show that BLEU is not a reliable indicator of functional correctness. 

\citet{ren2020codebleu} show that BLEU is not a reliable way of evaluating code.

\citet{austin2021program} also show that BLEU score is not reliable.

\citet{chen2021evaluating} provide a numerically stable implementation of pass@k.


\subsection{PL-to-PL translation}
Also know as answering the question of ``why is this easier than has been expected'', ``ML HAS been used to learn language to language translations'' and ``PL-to-PL is a hard problem, in general''

\citet{karaivanov2014phrase} use phrase-based statistical machine translation to do PL-to-PL translation. Their approach adds in understanding of the underlying PL grammar to guide the prefix generation process. They provide an example of C\# to Java.

\citet{allamanis2018survey} tells us what was done before 2018. Makes important statements about what this problem looks like from the PL/SE side.



==> very-big-table.tex <==
   \begin{xltabular}{0.99\textwidth}{l l l l *{9}{C} }\hline
         &&&& \multicolumn{2}{c}{\textsc{\textbf{Model}}} & \multicolumn{2}{c}{\textsc{\textbf{Temp}}} & \multicolumn{3}{c}{\textsc{\textbf{Docstrings}}} & \multicolumn{2}{c}{\textsc{\textbf{Terms}}}\\
         \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-11}\cmidrule(lr){12-13}
         \textsc{\textbf{PL}} & \textsc{$1$} & \textsc{$10$} & \textsc{$100$}& \emph{Codex}&\emph{Incoder}&\emph{0.2}&\emph{0.8}&\emph{Keep}&\emph{Remove}&\emph{Modify}&\emph{Keep}&\emph{Modify}\\\hline
         \endhead
          Bash&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform
              
         C++&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform
        
        C\#&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform
         D&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform
              
         Go&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
               
         Java&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
        
       JavaScript&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
              
         Julia&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
      
         Lua&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
              
      Perlt&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform      
      
       PHP&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
    
       R&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
    
       Racket&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
         
       Ruby&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform      
         
       Rust&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform  
    
       Scala&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
              
       Swift&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\ %incoder-0.8-transform-transform 
    
       Typescript&&&&$\times$&&$\times$&&$\times$&&&$\times$&\\ %davinci-0.2-keep-keep
              &&&&$\times$&&$\times$&&&&$\times$&&$\times$\\ %davinci-0.2-transform-transform
              &&&&$\times$&&$\times$&&&$\times$&&$\times$&\\ %davinci-0.2-remove-keep
              &&&&$\times$&&$\times$&&&&$\times$&$\times$&\\ %davinci-0.2-transform-keep
              &&&&$\times$&&&$\times$&$\times$&&&$\times$&\\ %davinici-0.8-keep-keep
              &&&&$\times$&&&$\times$&&&$\times$&&$\times$\\ %davinci-0.8-transform-transform
              &&&&&$\times$&$\times$&&$\times$&&&$\times$&\\ %incoder-0.2-keep-keep
              &&&&&$\times$&$\times$&&&&$\times$&&$\times$\\ %incoder-0.2-transform-transform
              &&&&&$\times$&$\times$&&&$\times$&&$\times$&\\ %incoder-0.2-remove-keep
              &&&&&$\times$&$\times$&&&&$\times$&$\times$&\\ %incoder-0.2-transform-keep
              &&&&&$\times$&&$\times$&$\times$&&&$\times$&\\ %incoder-0.8-keep-keep
              &&&&&$\times$&&$\times$&&&$\times$&&$\times$\\\hline %incoder-0.8-transform-transform
               %\caption{This is the very big table} \label{tab:vbt}
    \end{xltabular}
   
